Self-Aware Feedback-Based Self-Learning in Large-Scale Conversational AI

Self-learning paradigms in large-scale conversational AI agents tend to leverage user feedback in bridging between what they say and what they mean. However, such learning, particularly in Markov-based query rewriting systems have far from addressed the impact of these models on future training where successive feedback is inevitably contingent on the rewrite itself, especially in a continually updating environment. In this paper, we explore the consequences of this inherent lack of self-awareness towards impairing the model performance, ultimately resulting in both Type I and II errors over time. To that end, we propose augmenting the Markov Graph construction with a superposition-based adjacency matrix. Here, our method leverages an induced stochasticity to reactively learn a locally-adaptive decision boundary based on the performance of the individual rewrites in a bi-variate beta setting. We also surface a data augmentation strategy that leverages template-based generation in abridging complex conversation hierarchies of dialogs so as to simplify the learning process. All in all, we demonstrate that our self-aware model improves the overall PR-AUC by 27.45%, achieves a relative defect reduction of up to 31.22%, and is able to adapt quicker to changes in global preferences across a large number of customers.

==> sections/future.tex <==
\section{Future Work}
\color{blue}
While the self-aware Markov model outperforms the vanilla baseline in terms of reactivity rate, it is still subject to some limitations as discussed in the Appendix Section \ref{appendix:risks}. We can further accelerate the pace of self-learning by incorporating time-based decays in the modeling process. 

In order to better handle tail traffic, we plan to personalize the Markov model. In such personalized settings, arbitrating between multiple potential rewrites and gathering evidence with sufficient statistics are some of the challenges to be overcome. Further, while our work currently focuses on Markov Graphs, the principles of self-awareness could also be extended to other modeling choices as well.
\color{black}
